RobustState: Boosting Fidelity of Quantum State Preparation via Noise-Aware Variational Training

Quantum state preparation, a crucial subroutine in quantum computing, involves generating a target quantum state from initialized qubits. Arbitrary state preparation algorithms can be broadly categorized into arithmetic decomposition (AD) and variational quantum state preparation (VQSP). AD employs a predefined procedure to decompose the target state into a series of gates, whereas VQSP iteratively tunes ansatz parameters to approximate target state. VQSP is particularly apt for Noisy-Intermediate Scale Quantum (NISQ) machines due to its shorter circuits. However, achieving noise-robust parameter optimization still remains challenging. We present RobustState, a novel VQSP training methodology that combines high robustness with high training efficiency. The core idea involves utilizing measurement outcomes from real machines to perform back-propagation through classical simulators, thus incorporating real quantum noise into gradient calculations. RobustState serves as a versatile, plug-and-play technique applicable for training parameters from scratch or fine-tuning existing parameters to enhance fidelity on target machines. It is adaptable to various ansatzes at both gate and pulse levels and can even benefit other variational algorithms, such as variational unitary synthesis. Comprehensive evaluation of RobustState on state preparation tasks for 4 distinct quantum algorithms using 10 real quantum machines demonstrates a coherent error reduction of up to 7.1 $\times$ and state fidelity improvement of up to 96\% and 81\% for 4-Q and 5-Q states, respectively. On average, RobustState improves fidelity by 50\% and 72\% for 4-Q and 5-Q states compared to baseline approaches.

==> figtex/learning_curve.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/learning_curve.pdf}
    % \vspace{-20pt}
    \caption{Training Curves of Four Different Tasks. From left to right: $4$ qubits and $5$ qubits on ibm\_hanoi with topology-aware CNOT ansatz; $4$ qubits and $5$ qubits with topology-aware native pulse ansatz on ibmq\_guadalupe. We train the ansatz on noise-free simulators for $500$ steps. Then we train for another $50$ steps with noise-aware loss generated from real machines. 
    \hl{The parameter are tuned according to real machine noise. Evaluated on real machines.}}
    \label{fig:learning_curve}
\end{figure*}


==> figtex/main_5q_4task.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main_5q_4task.pdf}
    % \vspace{-20pt}
    \caption{\name achieves the highest fidelity on various real machines using the topology-aware ansatz with \cnot\xspace gates for a number of 5-Q target states when compared with the Qiskit baseline. Evaluated on real machines.}
    \label{fig:main_5q_4task}
    % \vspace{-10pt}
\end{figure*}

==> figtex/main_5q_4task_pulse.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main_5q_4task_pulse.pdf}
    % \vspace{-20pt}
    \caption{On two machines with pulse supports, ibmq\_guadalupe and ibmq\_jakarta, \name, using topology-aware \rzx gates achieves the highest fidelity for various 5-Q states when compared with the Qiskit baseline. Evaluated on real machines.}
    \label{fig:main_5q_4task_pulse}
    % \vspace{-10pt}
\end{figure*}



==> figtex/metrology.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/metrology.pdf}
    % \vspace{-20pt}
    \caption{\hl{New figure. The accumulative minimal loss of two quantum state regression tasks, evaluated on real machines.}}
    \label{fig:metrology}
    % \vspace{-15pt}
\end{figure}


==> figtex/shadow_readout_mitigation.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/shadow_readout_mitigation.pdf}
    % \vspace{-20pt}
    \caption{Performance of three different tomography methods. We test three different tomography methods, our implementation of classical shadow tomography with and without readout error mitigation and the tomography implemented in Qiskit. We construct a $3$-Q random circuit and get its ideal density matrix $\rho$ in classical simulation. Then we perform the different tomography methods in a readout-error-only simulator with varying shots per measurement basis and get the estimated density matrix $\hat\rho$. We report the fidelity $F(\rho,\hat\rho)$ as the $y$ axis in the figure. The shaded area is $\pm 5$\x the standard deviation of the measured fidelity.}
    \label{fig:shadow_readout_mitigation}
    % \vspace{-10pt}
\end{figure}


==> figtex/unitary.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/unitary.pdf}
    % \vspace{-20pt}
    \caption{\hl{New figure. The accumulative maximal fidelity of two unitary synthesis tasks, evaluated in real machines, showing our framework can be used for other VQAs.}}
    \label{fig:unitary}
    % \vspace{-15pt}
\end{figure}


==> tables/tab_runtime.tex <==
\begin{table}[t]
\centering
\renewcommand*{\arraystretch}{1}
\setlength{\tabcolsep}{17pt}
\footnotesize
\caption{Circuit compilation & training time
}
\vspace{-8pt}

\begin{tabular}{lcccc}
\toprule
& Depth & \#Gates (\#1Q+\#CNOT) & \#Params & Acc. \\
\midrule
Noise-Unaware  & 237 & 365 (299+66) & 120 & 0.48 \\ 
\midrule
Random & 45 & 100 (94+6) & 36 & 0.86 \\
\midrule
Human & 64 & 135 (124+11) & 36 &  0.88 \\
\midrule
\textbf{\name} & 70 & 133 (123+10) & 36 & \textbf{0.89} \\
\midrule
\textbf{\ \ \ + Pruning} & 59 & 116 (106+10) & 22 & \textbf{0.92} \\
\bottomrule

\end{tabular}


\label{tab:depth}
\vspace{-15pt}

\end{table}
